Disentangling Decentralized Finance (DeFi) Compositions

We present a measurement study on compositions of Decentralized Finance protocols, which aim to disrupt traditional finance and offer services on top of distributed ledgers, such as Ethereum. DeFi compositions may impact the development of ecosystem interoperability, are increasingly integrated with web technologies, and may introduce risks through complexity. Starting from a dataset of 23 labeled DeFi protocols and 10,663,881 associated Ethereum accounts, we study the interactions of protocols and associated smart contracts. From a network perspective, we find that decentralized exchanges and lending protocols have high degree and centrality values, that interactions among protocol nodes primarily occur in a strongly connected component, and that known community detection methods cannot disentangle DeFi protocols. Therefore, we propose an algorithm to decompose a protocol call into a nested set of building blocks that may be part of other DeFi protocols. With a ground truth dataset we have collected, we can demonstrate the algorithm's capability by finding that swaps are the most frequently used building blocks. As building blocks can be nested, i.e., contained in each other, we provide visualizations of composition trees for deeper inspections. We also present a broad picture of DeFi compositions by extracting and flattening the entire nested building block structure across multiple DeFi protocols. Finally, to demonstrate the practicality of our approach, we present a case study that is inspired by the recent collapse of the UST stablecoin in the Terra ecosystem. Under the hypothetical assumption that the stablecoin USD Tether would experience a similar fate, we study which building blocks and, thereby, DeFi protocols would be affected. Overall, our results and methods contribute to a better understanding of a new family of financial products.

==> macros.tex <==
% !TeX root = main.tex

\RequirePackage{xspace,color}
\RequirePackage{tikz}
\RequirePackage{tikz-network}
\RequirePackage{makecell}
\RequirePackage{soul}

\RequirePackage{caption}
\RequirePackage{subcaption}


\usetikzlibrary{shapes.misc}

\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}


\newcommand\fix[1]{\textcolor{green}{#1}}
\newcommand\todo[1]{\textcolor{red}{TODO: #1}}
\newcommand\stefan[1]{\textcolor{blue}{Stefan: #1}}
\newcommand\pietro[1]{\textcolor{green}{Pietro: #1}}
\newcommand\bernhard[1]{\textcolor{green}{Bernhard: #1}}
\newcommand\friedhelm[1]{\textcolor{green}{Friedhelm: #1}}


\newcommand\revision[1]{\textcolor{black}{#1}}


% General

% DeFi stats
\newcommand{\DeFiTotalValue}{106\xspace}

\newcommand{\DeFiNumberProtocols}{\num{23}\xspace}
\newcommand{\DeFiNumberSeedAddr}{\num{1407}\xspace}
\newcommand{\DeFiNumberAccounts}{\num{10663881}\xspace}
\newcommand{\contractsNumber}{\num{46112390}\xspace}
\newcommand{\ERCNumber}{\num{324143}\xspace}

% time references
\newcommand{\TracesFrom}{01-Jan-2021 (block 11,565,019)\xspace} %\footnote{Jan-01-2021 12:00:00 AM +UTC}
\newcommand{\TracesTo}{05-Aug-2021 (block 12,964,999)\xspace} %\footnote{Aug-05-2021 12:33:32 PM +UTC}
\newcommand{\SeedFrom}{06-Mar-2021\xspace}
\newcommand{\SeedTo}{05-Aug-2021\xspace}

% common terms
\newcommand{\EOA}{\textit{EOA}\xspace} % externally owned account 
\newcommand{\EOAs}{\textit{EOAs}\xspace} % externally owned account plural
\newcommand{\CA}{\textit{CA}\xspace} % code account (= smart contract)
\newcommand{\CAs}{\textit{CAs}\xspace} % code account plural
\newcommand{\traces}{\textit{traces}\xspace} % raw trace data frame
\newcommand{\protocolTraces}{\textit{protocol traces}\xspace} % filtered traces where the external transcation goes to a protocol of our extended seed addresses
\newcommand{\protocolSubTraces}{\textit{protocol subtraces}\xspace} % filtered traces where the external transcation goes to a protocol of our extended seed addresses
\newcommand{\creationTraces}{\textit{creation traces}\xspace} % internal transactions where the transaction type is 'create'
\newcommand{\contracts}{\textit{contracts}\xspace} % contract data frame of all existing CAs and their ERC20 compability




